Fast and General Automatic Differentiation for Finite-State Methods

We propose a new method, that we coined the ``morphism-trick'', to integrate custom implementations of vector-Jacobian products in automatic differentiation softwares, applicable to a wide range of semiring-based computations. Our approach leads to efficient and semiring-agnostic implementations of the backward pass of dynamic programming algorithms. For the particular case of finite-state methods, we introduce an algorithm that computes and differentiates the $\oplus$-sum of all paths' weight of a finite-state automaton. Results show that, with minimal effort from the user, our novel library allows computing the gradient of a function w.r.t. to the weights of a finite state automaton orders of magnitude faster than state-of-the-art automatic differentiation systems. Implementations are made available via an open-source library distributed under a permissive license.

==> figures/cg_backward2.tex <==
\begin{forest}
    for tree={edge=-{Stealth}}
    [$\frac{\partial z}{\partial z_1}$
        [$\frac{\partial z_1}{\partial u_1}$, 
            [$\frac{\partial u_1}{\partial x_1}$]
            [$\frac{\partial u_1}{\partial y_1}$]
        ]
        [$\frac{\partial z_1}{\partial z_2}$,s sep=1cm
            [$\frac{\partial z_2}{\partial u_2}$
                [$\frac{\partial u_2}{\partial x_2}$]
                [$\frac{\partial u_2}{\partial y_2}$]
            ]
            [....
                [$\frac{\partial z_{K-2}}{\partial z_{K-1}}$,edge label={node[midway,right]{$\frac{\partial z_{...}}{\partial z_{...}}$}}
                    [$\frac{\partial z_{K-1}}{\partial u_{K-1}}$
                        [$\frac{\partial u_{K-1}}{\partial x_{K-1}}$]
                        [$\frac{\partial u_{K-1}}{\partial y_{K-1}}$]
                    ]
                    [$\frac{\partial z_{K}}{\partial u_{K}}$
                        [$\frac{\partial u_{K}}{\partial x_K}$]
                        [$\frac{\partial u_K}{\partial y_K}$]
                    ]
                ]
            ]
        ]
    ]
\end{forest}

==> figures/cg_backward_flat2.tex <==
\begin{forest}
    for tree={edge=-{Stealth}}
    [$\frac{\partial z}{\partial \mu(z)}$
        [$\frac{\partial \mu(u_1)}{\partial u_1}$, 
            [$\frac{\partial u_1}{\partial x_1}$]
            [$\frac{\partial u_1}{\partial y_1}$]
        ]
        [....]
        [$\frac{\partial \mu(u_K)}{\partial u_K}$, 
            [$\frac{\partial u_K}{\partial x_K}$]
            [$\frac{\partial u_K}{\partial y_K}$]
        ]
    ]
\end{forest}

==> figures/cg_forward2.tex <==
\begin{forest}
    for tree={edge={Stealth}-,l sep=1cm}
    [$\oplus$
        [$\otimes$, 
            [$x_1$]
            [$y_1$]
        ]
        [$\oplus$,s sep=1cm
            [$\otimes$
                [$x_2$]
                [$y_2$]
            ]
            [....
                [$\oplus$
                    [$\otimes$
                        [$x_{K-1}$]
                        [$y_{K-1}$]
                    ]
                    [$\otimes$
                        [$x_K$]
                        [$y_K$]
                    ]
                ]
            ]
        ]
    ]
\end{forest}
